Near-optimal-sample estimators for spherical Gaussian mixtures

Statistical and machine-learning algorithms are frequently applied to high-dimensional data. In many of these applications data is scarce, and often much more costly than computation time. We provide the first sample-efficient polynomial-time estimator for high-dimensional spherical Gaussian mixtures. For mixtures of any $k$ $d$-dimensional spherical Gaussians, we derive an intuitive spectral-estimator that uses $\mathcal{O}_k\bigl(\frac{d\log^2d}{\epsilon^4}\bigr)$ samples and runs in time $\mathcal{O}_{k,\epsilon}(d^3\log^5 d)$, both significantly lower than previously known. The constant factor $\mathcal{O}_k$ is polynomial for sample complexity and is exponential for the time complexity, again much smaller than what was previously known. We also show that $\Omega_k\bigl(\frac{d}{\epsilon^2}\bigr)$ samples are needed for any algorithm. Hence the sample complexity is near-optimal in the number of dimensions. We also derive a simple estimator for one-dimensional mixtures that uses $\mathcal{O}\bigl(\frac{k \log \frac{k}{\epsilon} }{\epsilon^2} \bigr)$ samples and runs in time $\widetilde{\mathcal{O}}\left(\bigl(\frac{k}{\epsilon}\bigr)^{3k+1}\right)$. Our other technical contributions include a faster algorithm for choosing a density estimate from a set of distributions, that minimizes the $\ell_1$ distance to an unknown underlying distribution.

==> commentedstuff.tex <==

Applying bounds on $n$ results in the lemma.
%\begin{equation}
%\label{eq1}
%\max \left( \frac{|\mup_i- \muq_i|}{\max(\sigp_i,\sigq_i)},   \frac{|\sigp^2_i -\sigq^2_i +\mup^2_i -\muq^2_i|}{\max(\sigp^2_i,\sigq^2_i)} \right).
%\end{equation}
%For this co-ordinate let $\frac{|\mup_i- \muq_i|}{\max(\sigp_i,\sigq_i)} $ be the term that maximizes the about quantity.
%If we know $\wmup_i$ and $\wmuq_i$ extactly then the above term gives us $\wmup_j - \wmuq_j$ for all $j \neq i$.
%But since we are dividing the error by $\mup'_i - \wmuq'_i$ instead of $\wmup_i-\wmuq_i$, the error in finding $\wmup_j-\wmuq_j$ is
%\begin{align*}
%|\wmup_j - \wmuq_j -(\mup'_j-\muq'_j)| 
%&\leq |\wmup_j-\wmuq_j|\frac{3\max(\sigp_i,\sigq_i) \sqrt{2 \log d/\delta}}{\gamma \sqrt{n\min(\wwp,\wwq)}} \\
%& \leq \frac{3\max(\sigp_j,\sigq_j) \sqrt{2 \log d/\delta}}{ \sqrt{n\min(\wwp,\wwq)}} 
%\end{align*}
%The second inequality follows from the fact that co-ordinate $i$ achieved the maximum in Equation~\eqref{eq1}.
%By Lemma~\ref{??}, 
%\[
%|\wmup_j - \wmuq_j -(\mup_j-\muq_j)| \leq \frac{7 \max(\sigp_j,\sigq_j) \log \frac{1}{\delta}}{n\min(\wwp,\wwq)}.
%\]
%Once we solve the equations, we get the error for $\mup_j$ as
%\[
%|\mup'_j -\mup_j|\leq \frac{7 \max(\sigp_j,\sigq_j) \log \frac{1}{\delta}}{n} \biggl( 1 + \frac{\wwq}{\sqrt{\min(\wwp,\wwq)}} \biggr).
%\]
%we show that $\wmup_j -\wmuq_j$ is estimated with error at most $ $.
%
%Together with $ $, this implies the result.


\begin{center}
\fbox{\begin{minipage}{1.0\textwidth}
Algorithm \textsc{Learn $2$-Gaussian oriented} \newline
\textbf{Input:} $U$ a set of $n$ samples from $\fvec$ and $\epsilon$
\begin{enumerate}
%\item Compute the empirical mean $\wmur$ and variance $\wsigr^2$
\item[] For all co-ordinates $i$ do:
\item let $A = \{-\infty,\xvec_i(1),\xvec_i(2), \ldots,\xvec_i(n), \infty\}$. For every pair of points $a,b \in A$
let $U'$ be the set of samples such that $\xvec_i(j) \in [a,b]$. Let $U' = \argmax (|U'|,|U \setminus U'|)$. For all $U'$ do:
\item Let $\wwp$ and $\wwp'$ be the empirical occurances of $\pvec$ in mixtures $U$ and $U'$ respectively. 
For $\wwp = l/n : 1 \leq l \leq |U|$ and $\wwp' = l/|U'|: 1 \leq l \leq |U'|$ do:
\begin{itemize}
  \item For all $j \neq i$, solve $\wwp \wmup_j + \wwq \wmuq_j =\wmur_j$ and 
$\wwp' \wmup_j + \wwq' \wmuq_j =\wmur'_j$.
  \item For all $j \neq i$, solve $\wwp(\wsigp^2_j +\wmup^2_j)+ \wwq (\wsigq^2_j +\wmuq^2_j) = \wmur^2_j + \wsigr^2_j$ and 
  $\wwp'(\wsigp'^2_j +\wmup'^2_j)+ \wwq (\wsigq'^2_j +\wmuq'^2_j) =\wmur^2_j + \wsigr^2_j$.
  \item Generate a list of candidate parameters for co-ordinate $i$ using in Lemma~\ref{lem:coolsearch} such that one of them 
  satisfies $\wp\lone{p_i}{\hat{p_i}} + \wq\lone{q_i}{\hat{q_i}} \leq \epsilon/4$.
 \item For all possible parameters for co-ordinate $i$ from the previous step, and estimates for $j \neq i$, run \textsc{cluster}$(\wwp,\wpvec,\wqvec)$.
 \end{itemize}
 \end{enumerate}
\end{minipage}}
\end{center}

\begin{center}
\fbox{\begin{minipage}{1.0\textwidth}
Subroutine algorithm \textsc{Cluster} \newline
\textbf{Input: } Estimates $(\wwp,\wpvec$,$\wqvec)$, 
$n$ samples from $\fvec$, and $\alpha$(a constant calculated later in the proofs)
\begin{enumerate} 
\item For all $i$, use $n$ samples to estimate  $\wsigl_i$ be the largest separation between two samples in co-ordinate $i$ and $\wsigs_i$ be the shortest width of $n\min(\wwp,\wwq)$ contiguous points.
Discard those samples.
\item Repeat the following steps by changing $\pvec$ to $\qvec$.
\begin{itemize}
\item Find sets  $\bpmg = \{i :  \wmup_i - \wmur_i \geq \wsigl \alpha,\}$,
$\bpml = \{i:  \wmup_i - \wmur_i \leq \wsigl \alpha,\}$, and $\bpv = \{i \in [d] \setminus (\bpmg \cup \bpml): (\wmup^2_i +\sigp^2_i) \leq  (\wmur^2_i +\sigr^2_i) + \alpha \wsigl^2_i \}$. 
\item Use single-linkage to cluster samples  with metric $\sum_{i \in \bpmg} X_i/\wsigl_i$ and compute empirical averages within the clusters
and include it in $\cF$. 
%with $\cF = \cF \cup \{(\wpvec',\wqvec',\wwp)\}$
\item Repeat the single linkage algorithm with metric $\sum_{i \in \bpv} X^2_i/\wsigl^2_i$ and metric $\sum_{i \in \bpml} X_i/\wsigl_i$.
\end{itemize}
\item Let $B = \bpmg \cup \bpml \cup \bpv \cup \bqmg \cup \bqml \cup \bqv$.
\item If $\min(\wwp,\wwq) \leq \epsilon/3|B|$
\begin{itemize}
 \item Use Lemma~\ref{lem:coolsearch} to change the estimate for co-ordinates $B$.
 \end{itemize}
 \item If $\min(\wwp,\wwq) \geq \epsilon/3|B|$
 \begin{itemize}
\item For co-ordinates in $B$ such that $\wsigp^s_i \leq \wsigq^l_i \epsilon_1$ learn density in those co-ordinates using Lemma~\ref{lem:coolsearch} 
to accuracy $\epsilon_1$. 
\item If $|\wwp - 1/2| \leq \epsilon_1$. Use an iterative Scheffe as described in Lemma~\ref{lem:itscheffe} to associate parameters 
to the component and update the parameters for co-ordinates such that  $\wsigp^s_i \leq \wsigq^l_i \epsilon_1$. Include the mixture to $\cF$.
\end{itemize}
\end{enumerate}
\end{minipage}}
\end{center}


\begin{Lemma}
\label{lem:sigsbound}
Let $\sigs_i = \min(\sigp_i,\sigq_i)$. If $ n\min(\wp,\wq) \geq 100\log n/\delta$, then
With probability $\geq 1-\delta$, for all co-ordinates $i$,
 \[
  \sigs_i \leq \wsigs_i \leq 10\sigs_i \sqrt{\log n/\delta}.
 \]
\end{Lemma}
\begin{proof}
Since $ n\min(\wp\wq) \geq 100\log n/\delta$, by Chernoff bounds 
 $n \min(\wwp,\wwq)\geq 10 \log n/\delta$. For every sample probability that $\geq 10 \log n/\delta$ samples
occuring in the interval $\leq \sigs_i$ is $\leq \delta/n$. Hence by the union bound $\wsigs_i \geq \sigs_i$.

Let $p$ be the distribution with least variance in co-ordinate $i$. Since $n\wwp \geq n \min(\wwp,\wwq)$, 
$\wsigs_i$ is less than the distance between $n\wwp$ contiguoous points. However since there are $n\wwp$ points from $\pvec$,
their distance is $\leq 10\sigs_i \sqrt{\log n/\delta}$.
\end{proof}


\vspace{-2ex}
\begin{center}
\fbox{\begin{minipage}{1.0\textwidth}
Subroutine algorithm \textsc{Cluster} \newline
\textbf{Input: } Estimates $(\wwp,\wpvec$,$\wqvec)$, 
$n$ samples from $\fvec$, and $\alpha$(a constant calculated later in the proofs)
\begin{enumerate} 
\item and $\wsigs_i$ be the shortest width of $n\min(\wwp,\wwq)$ contiguous points.
Discard those samples.
\item Repeat the following steps by changing $\pvec$ to $\qvec$.
\begin{itemize}
\item Find sets  $\bpmg = \{i :  \wmup_i - \wmur_i \geq \wsigl \alpha,\}$,
$\bpml = \{i:  \wmup_i - \wmur_i \leq \wsigl \alpha,\}$, and $\bpv = \{i \in [d] \setminus (\bpmg \cup \bpml): (\wmup^2_i +\sigp^2_i) \leq  (\wmur^2_i +\sigr^2_i) + \alpha \wsigl^2_i \}$. 
\item Use single-linkage to cluster samples  with metric $\sum_{i \in \bpmg} X_i/\wsigl_i$ and compute empirical averages within the clusters
and include it in $\cF$. 
%with $\cF = \cF \cup \{(\wpvec',\wqvec',\wwp)\}$
\item Repeat the single linkage algorithm with metric $\sum_{i \in \bpv} X^2_i/\wsigl^2_i$ and metric $\sum_{i \in \bpml} X_i/\wsigl_i$.
\end{itemize}
\item Let $B = \bpmg \cup \bpml \cup \bpv \cup \bqmg \cup \bqml \cup \bqv$.
\item If $\min(\wwp,\wwq) \leq \epsilon/3|B|$
\begin{itemize}
 \item Use Lemma~\ref{lem:coolsearch} to change the estimate for co-ordinates $B$.
 \end{itemize}
 \item If $\min(\wwp,\wwq) \geq \epsilon/3|B|$
 \begin{itemize}
\item For co-ordinates in $B$ such that $\wsigp^s_i \leq \wsigq^l_i \epsilon_1$ learn density in those co-ordinates using Lemma~\ref{lem:coolsearch} 
to accuracy $\epsilon_1$. 
\item If $|\wwp - 1/2| \leq \epsilon_1$. Use an iterative Scheffe as described in Lemma~\ref{lem:itscheffe} to associate parameters 
to the component and update the parameters for co-ordinates such that  $\wsigp^s_i \leq \wsigq^l_i \epsilon_1$. Include the mixture to $\cF$.
\end{itemize}
\end{enumerate}
\end{minipage}}
\end{center}




We now state a simple lemma about single-linkage clustering. The proof follows from 
tiangle inequality and union bound.
\begin{Lemma}
\label{lem:singlelink}
 Consider a single linkage algorithm for two distributions $p$ and $q$ using metrix $Y$. If the difference in means of $Y$ is $\geq 3t$
 and for any sample from $p$ and $q$, $\Pr(|Y - \EE[Y]| \geq t) \leq \delta/2n$. Then,
 the single linkage algorithm clusters all samples correctly with error $\leq \delta$.
\end{Lemma}


We now show that if the weight of a component is small and corresponding sets $B$ is large then the algorithm \textsc{cluster},
clusters them into two groups effectively and thus learns them.
\begin{Lemma}
If $\wp \geq \epsilon$ and $|\bpmg| \geq 10 \alpha^{-1} \log n/\delta$, then after \textsc{cluster},
$\cF$ contains a mixture $\epsilon$ close to $\fvec$ with probability $\geq 1-4 \delta$.
Similar result holds for $\bpml$, $\bqmg$, and $\bqml$.
\end{Lemma}
\begin{proof}
If $\wp \geq \epsilon/2$, then by Lemma~\ref{lem:lineq}, and its proof,
\[
 |\wmup_i -\wmur_i - (\mupi-\mur_i)|  \leq \sigl/\sqrt{10d}. 
\]
By Lemma~\ref{lem:siglbound}, $\wsigl \geq \sigl$. Hence, $|\mupi - \mur_i| \geq \alpha \wsigl/2$.
Furthermore,
\[
\mup_i - \muq_i \geq \mup_i - \mur_i  \geq \alpha \wsigl_i/2.
\]
% Hence, if $|\wmup_i -\wmur_i| \geq \alpha \wsigl$ and then 
% \[
% |\wmup_i -\wmur_i| \geq \alpha \wsigl.
% \]
Now consider the quantity, $\sum_{i \in \bpm} X_i/\wsigl_i$. For both $\pvec$ and $\qvec$ 
these are Gaussians with difference in means in both cases being $|\bpm|\alpha$ and variance 
$|\bpm|$. Therefore with $|\bpm| \geq 10 \alpha^{-1}\log n/\delta$, samples concentrate around mean with error $\leq \delta/n$.
Then by Lemma~\ref{lem:singlelink},
samples are clustered correctly with error $\leq \delta$.
% then by Lemma~\ref{lem:gaussbound},
% similar to the other proofs of single-linkage clustering, the samples are clustered such that there is no mis-clustering.
Therefore by Lemma~\ref{lem:withinclus}, $\cF$ includes an $\epsilon$-close mixture to $\fvec$.
By the union bound the error is $\leq 4\delta$.
\end{proof}

\begin{Lemma}
If $\wp\geq \epsilon/2$ and $|\bpv| \geq 100\alpha^{-1} \log n/\delta$, then with probability $\geq 1-3\delta$,
\textsc{cluster} returns correct clusters.
\end{Lemma}
\begin{proof}
 If $\wp \geq \epsilon/2$, then by Lemma~\ref{lem:lineq}, and its proof,
\[
 |\sigp^2_i + \mup^2_i - (\wsigp^2_i + \wmur^2_i) |  \leq \sigl^2/2\sqrt{10d}. 
\]
Simiarly by the proof of Lemma~\ref{lem:lineq}
\[
 |\wsigr^2 + \wmur^2 - \wwp (\sigp^2_i + \mup^2_i) - \wwq (\sigq^2_i + \muq^2_i)| \leq \sigl^2/2\sqrt{10d}.
\]
By Lemma~\ref{lem:siglbound}, $\wsigl \geq \sigl$. Hence, $|\sigp^2_i + \mup^2_i - \sigq^2_i + \muq^2_i| \geq \alpha \wsigl^2/2$.
Now consider the quantity $\sum_{i \in \bpv} X^2_i/\wsigl^2_i$. For both samples from $\pvec$ and $\qvec$ they are sum of weighted
squared Gaussians. Since, $|\sigp^2_i + \mup^2_i - \sigq^2_i + \muq^2_i| \geq \alpha \wsigl^2/2$,
the difference in expections is $\geq |\bpv|\alpha/2$. To prove the concentration, consider samples from $p_i$,
\[
 \sum_{i \in \bpv} \frac{X^2_i}{\wsigl^2_i} =  \sum_{i \in \bpv} \frac{(X_i -\mup_i)^2 + \mup_i^2 + \mup_i(X_i -\mup_i)}{\wsigl^2_i}.
\]
The first term  $\sum_{i \in \bpv} \frac{(X_i -\mup_i)^2}{\wsigl^2_i}$ is same as
sum of $|\bpv|$ standard normal distributions with weights $\sigl^2/\wsigl^2 \leq 1$ and hence, by Lemma~\ref{lem:tailchi},
with probability $\geq 1-\delta$ it concentrates around the mean by $\sqrt{|\bpv|\log d/\delta}$.
Simiarly the last term $ \sum_{i \in \bpv} \frac{\mup_i(X_i -\mup_i)}{\wsigl^2_i}$ is a Gaussian distribution with mean $0$ and variance 
$\leq |\bpv|$ and hence concentrates around its mean with error $\sqrt{|\bpv|\log d/\delta}$ with probability $\geq 1-\delta$.
Hence, by Lemma~\ref{lem:singlelink}, the sampls are clustered properly. Therefore by Lemma~\ref{lem:withinclus}, $\cF$ includes an $\epsilon$-close mixture to $\fvec$.
By the union bound the error is $\leq 4\delta$.
\end{proof}

\begin{Lemma}
If $\alpha \leq 1/100(\log n/\delta)$ and $\wp \geq \epsilon/2$, then with probability $\geq 1-4\delta$, in $[d]\setminus B$,  $\sigp/\sigl \geq 1/2$.
\end{Lemma}
\begin{proof}
 Consider the term $(\mup_i - \muq_i)^2$. Since $i \nin B$, $|\wmup_i-\wmur_i| \leq \alpha \wsigl_i$. However by Lemma~\ref{lem:lineq}
 and its proof $|\mupi -\mur_i -(\wmup_i - \wmur_i)| \leq 1/20\sqrt{d}$, hence $|\mup_i -\wmur_i| \leq \alpha \wsigl_i/2$ and hence
 $|\mup_i - \wmuq_i| $
\end{proof}


\begin{Lemma}
 Consider two one dimensional mixtures $f$ and $f'$ with the same mixing weights such that $\lone{f}{f'} \leq \epsilon_1$. 
 Let $\min(\wp,\wq) \geq \epsilon_2$ and $\min(\sigp,\sigq)/\max(\sigp,\sigq) \leq \epsilon_1 < \epsilon_2$,
 then $\lone{p}{p'} \leq \epsilon_1/\epsilon_2$.
\end{Lemma}
\begin{proof}
 Since $\lone{f}{f'} \leq \epsilon_1$, given $1/\sqrt{\epsilon_1}$ samples they cannot be distinguished with probability $ \geq 1/10$.
Therefore if we look at the maximum separation between two samples, they are same for both the mixtures, therefore 
$\max(\sigp $. Consider the set $A$ where $p(x) \geq q(x)$, Since $\lone{p}{q} \geq -\epsilon_1/2$. $q$ assigns probability and
Since $\sigq'$ is also large, $q'(A)$ is also small. Therefore $p'(A)$ is large and hence $\lone{p}{p'} \leq \epsilon_1/wp$.
Therefore $p'(A^c) \leq \epsilon_1$ and hence $\lone{q}{q'} \leq \epsilon_1$.
\end{proof}



%
%\begin{center}
%\fbox{\begin{minipage}{1.0\textwidth}
%Algorithm \textsc{Learn $2$-Gaussian oriented} \newline
%\textbf{Input:} $n$ samples from $\fvec$ and $\epsilon$
%\begin{enumerate}
%\item Compute the empirical mean $\wmur$ and variance $\wsigr^2$
%\item For every pair of co-ordinates compute $\hat{\EE}[X_i X_j]$, $\hat{\EE}[X^2_iX_j]$, and $\hat{\EE}[X^2_iX^2_j]$ 
%\item For all co-ordinates $i$, for $\wmup_i,\sqrt{\wmup^2_i+\wsigp^2_i} \in \Xvec(j)_i: 1\leq j \leq n$ $\wwp = j/n : 1 \leq j \leq n$ do:
%\item[] \textbf{Far means:}
%\begin{itemize}
%  \item Compute $\wmuq_i$ and $\sqrt{\wmup^2_i+\wsigp^2_i}$ by solving $\wwp \wmup_i + \wwq \wmuq_i =\wmur_i$ and 
%  $\wwp(\wmup^2_i+\wsigp^2_i) + \wwq (\wmuq^2_i+\wsigq^2_i) = \wsigr^2_i + \wmur^2_i$.
% \item For all $j \neq i$, solve  $\wmup_j - \wmuq_j = (\hat{\EE}[X_i X_j] - \wmur)/(\wmup_i -\wmuq_i)$ and $\wwp \wmup_j + \wwq \wmuq_j = \wmur$
% \item For all $j \neq i$, solve  $\wsigp^2_j +\wmup^2_j- \wsigq^2_j -\wmuq^2_j = (\hat{\EE}[X_i X^2_j] - \wsigr^2)/(\wmup_i -\wmuq_i)$ and $\wwp \wsigp^2 + \wwq \wsigq^2_j = \wsigr^2$
% \item $\cF = \cF \cup \{\wwp, \wpvec,\qvec\} $ and run \textsc{cluster}$(\wwp,\wpvec,\qvec)$
% \end{itemize}
% \item[] \textbf{Far variances:}
% \begin{itemize}
%  \item For all $j \neq i$, solve  $\wmup_j - \wmuq_j = (\hat{\EE}[X^2_i X_j] - \wmur)/(\wmup^2_i+\wsigp^2_i -\wmuq^2_i-\wsigq^2_i)$ and $\wwp \wmup_j + \wwq \wmuq_j = \wmur$
% \item For all $j \neq i$, solve  $\wsigp^2_j +\wmup^2_j- \wsigq^2_j -\wmuq^2_j = (\hat{\EE}[X^2_i X^2_j] - \wsigr^2)/((\wmup^2_i+\wsigp^2_i -\wmuq^2_i-\wsigq^2_i)$ and $\wwp \wsigp^2 + \wwq \wsigq^2_j = \wsigr^2$
% \item $\cF = \cF \cup \{\wwp, \wpvec,\qvec\} $ and run \textsc{cluster}$(\wwp,\wpvec,\qvec)$
%\end{itemize}
% \end{enumerate}
%\end{minipage}}
%\end{center}



\begin{Lemma}
\label{lem:yspeconc}
Let $Y(1), Y(2) \ldots Y(n)$ be samples from the mixture of a product distribution. If $Y$ satisfies properties
in Definition~\ref{def:good}, then the top eigenvector $\uvec$ of the sample covariance matrix without the diagonal entries
Let $A = \wp\wq\norm{\mup-\muq}^2$, then 
satisfy 
\[
\lV \uvec \cdot \frac{\mup(Y)-\muq(Y)}{\norm{\mup-\muq}} \rV \geq  
\]
\end{Lemma}
\begin{proof}
Let $\muave$ be the average of $Y$. By Lemma~\ref{lem:exp} for two components,
\begin{align*}
\frac{1}{n}\sum^n_{i=1} (Y(i)-\wmuave)(Y(i)-\wmuave)^t\\=  \sum^2_{i=1} \wwi(\wmupi-\wmuave)(\wmupi-\wmuave)^t -  \wwi(\wmupi-\mupi)(\wmupi-\mupi)^t + 
  \sum^k_{i=1}  \sum_{j | Y(j) \sim p_i}  \frac{1}{n}(Y(j)-\mupi)(Y(j)-\mupi)^t.
\end{align*}
Since the number of components $k=2$ and $p_1=p$ and $p_2=q$, we get 
$ \sum_{i=1} \wwi(\wmup-\wmuave)(\wmup-\wmuave)^t = 2\wwp\wwq(\wmup -\wmuq)(\wmup - \wmuq)^t$.

By Definition~\ref{def:well}, $\norm{\sum^2_{i=1} \wwi(\wmupi-\mupi)(\wmupi-\mupi)^t} \leq \sum^2_{i=1} \norm{\wmupi -\mupi}^2$.

By Theorem~\ref{thm:matconc}, the last term without the diagonal terms is bounded by
  \[
  \sum^k_{i=1}  \wwi  \leq
  \]
\end{proof}



\begin{proof}
 
\end{proof}



If either $\sum^d_{i=1} \frac{(\mup_i-\muq_i)^2}{\sigr^2_i}$ or $\sum^d_{i=1} \frac{(\sigp^2_i-\sigq^2_i+\mup^2_i-\muq^2_i)^2}{\sigr^4_i}$
is bigger than $  $, t

 \[
\sum^d_{i=1} \frac{(\mup_i-\muq_i)^2}{\sigr^2_i}  + \frac{(\sigp^2_i-\sigq^2_i+\mup^2_i-\muq^2_i)^2}{\sigr^4_i}  \geq \frac{\epsilon^2}{1280\wp^2\wq^2}.
 \]
\begin{Lemma}
\begin{itemize}
Let $\gamma \leq \epsilon^2/5000$ and $n \geq $
\item If $\sum^d_{i=1} \wp^2 \wq^2 \frac{(\mup_i-\muq_i)^2}{\sigr^2_i} \geq 1/5000$, then $\uvec \cdot \dvecm \geq $.
\item If $\sum^d_{i=1} \wp^2 \wq^2 \frac{(\sigp^2_i-\sigq^2_i+\mup^2_i-\muq^2_i)^2}{\sigr^4_i} \geq 1/5000$, then $\uvec \cdot \dvecv \geq $
\end{itemize}
\end{Lemma}
We now consider clustering of two product distribution that satisfy $n \geq $

Since we are searching over all values of $\alpha_i$ to an accuracy of $\epsilon_1$, there exists a set such that
for all $i$, $|\alpha_i -\alpha'_i| \leq \epsilon_1$.
Therefore,
\[
\frac{\mupi-\muave(C)}{\norm{\mupi -\muave(C)}} = \sum^{k-1}_{i=1} \alpha'_i \vvec_i + \sqrt{1-\norm{\alpha}^2} \vvec' + \sqrt{k\epsilon_1}^2 \vvec'',
\]
where $\vvec''$ is some vector in span of $\vvec_i$s.
We know that for components within each cluster $\sqrt{\wi} \norm{\mupi-\muave(C)} \leq 3\sigma k\sqrt{log n^2/\delta}$.
Therefore, if $\wi \geq \epsilon/4k$, then
$\norm{\mupi-\muave(C)} \leq 3\sigma k^{3/2}\sqrt{\epsilon^{-1/2}log n^2/\delta}$.
Hence,
\[
\mupi-\muave(C) = \norm{\mupi-\muave(C)} \sum^{k-1}_{i=1} \alpha'_i \vvec_i + \beta\vvec''',
\]
where $|\beta| \leq  3\sigma k^{3/2}\sqrt{\epsilon^{-1/2}log n^2/\delta}\sqrt{k\epsilon^2_1 + 1 - \norm{\alpha}^2}$.
Since we are searching over gridded values of $\norm{\mupi-\muave(C)}$ with accuracy $\epsilon_2$ we get that there is a vector over the search
such that $ |\mupi-\muave(C) - \uvec| \leq \epsilon_2 + 3\sigma k^{3/2}\sqrt{\epsilon^{-1/2}log n^2/\delta}\sqrt{k\epsilon^2_1 + 1 - \norm{\alpha}^2}$.




By Lemma~\ref{lem:searchexisits}, there is a vector that is $\epsilon \sigma$ close to $\mupi-\muave(C)$,
hence we have
\[
\wwi \norm{\mupi - \wmupi}^2 \leq \wwi \norm{\muave(C)-\wmuave(C)}^2 + \wwi \norm{\mupi-\muave(C) - \wmupi - \wmuave(C)}^2 \leq \epsilon^2/8k^2.
\]
Hence for each $j$ we have
\[
\wwi^2 \lone{\pvec_j}{\wpvec_j}^2 \leq \epsilon^2/4k^2.
\]
Summing over all the components yields the desired result.

We have clusters such that within each cluster the 




==> future.tex <==
\section{Conclusions and future work}
We have shown that mixtures of spherical Gaussians can be learned with near-linear number of samples in polynomial time.
While the sample complexity is near-optimal in terms of $d$, there is a factor of $k^9$ 
in terms of number of components. It would be interesting to reduce the polynomial dependence on $k$ or to find non-trivial lower bounds
on the number of samples in terms of $k$.
% 
% While extending this result to general mixtures remains a grandeur goal, we have some preliminary results to show that
% mixtures of two product distributions (Discrete, Poisson, Gaussian etc.) can be learnt in polynomial time in near-linear number of samples.
% \begin{Theorem}
% \label{thm:twoproduct}
% If  $n \geq c  \frac{d\log^8 (d/\delta) }{\epsilon^{8}}$ for some constant $c$, then there is a polynomial time algorithm that 
% with probability $\geq 1- \delta$, returns mixture is $\epsilon$-close to $\fvec$.
% The run time of the algorithm is $\tcO(d^7)$.
% \end{Theorem}
% The algorithm is a requires additional tools and analysis and we will include in subsequent paper.
